Distributed Online Big Data Classification Using Context Information

Distributed, online data mining systems have emerged as a result of applications requiring analysis of large amounts of correlated and high-dimensional data produced by multiple distributed data sources. We propose a distributed online data classification framework where data is gathered by distributed data sources and processed by a heterogeneous set of distributed learners which learn online, at run-time, how to classify the different data streams either by using their locally available classification functions or by helping each other by classifying each other's data. Importantly, since the data is gathered at different locations, sending the data to another learner to process incurs additional costs such as delays, and hence this will be only beneficial if the benefits obtained from a better classification will exceed the costs. We model the problem of joint classification by the distributed and heterogeneous learners from multiple data sources as a distributed contextual bandit problem where each data is characterized by a specific context. We develop a distributed online learning algorithm for which we can prove sublinear regret. Compared to prior work in distributed online data mining, our work is the first to provide analytic regret results characterizing the performance of the proposed algorithm.

==> cascaded.tex <==
\section{Online Learning in Cascaded Classifier Systems}

Different from the previous sections, in this section I assume that the classifiers are cascaded. The goal is to make a correct classification in a delay sensitive environment. When an input data stream arrives, it is forwarded to one of ${\cal M}$ classifiers. The classifier has three options. It can label the data as {\em classified} and return the label, label it as {\em irrelevant} and discard it, or label it as {\em further investigation is needed} and send it to another classifier. 

The goal is to learn which classification order is optimal for each arriving data $x(t)$. Note that there are $M!$ classification orders for each data, therefore even the optimization problem is very difficult to solve. However, it can be solved easily in an online setting. The learning algorithm choses an order $\sigma(1), \sigma(2), \ldots, \sigma(M)$ at each time step. For instance assume that for data input $x$, $\sigma(1), \sigma(2)$ is an optimal order. After a {\em classified} decision by the second classifier in the chain, the server not only updates the reward of the classification order $\sigma(1), \sigma(2), \ldots, \sigma(M)$, but it can update the rewards of all classification orders starting with $\sigma(1), \sigma(2)$. If you think of each arm as a classification order, then this learning problem exploits the correlation between the arms. I also propose to use a zooming type algorithm here. By this we don't have to worry about how the data arrives. 

We can also explore more complex classifier structures such as chains of classifiers working in parallel with different input data streams, but they can call each other sometimes to benefit from experience of other classifiers. 

==> centralized.tex <==
\section{An Optimal Classification Scheme with Perfect Information} \label{sec:centralized}

Our benchmark when evaluating the performance of the learning algorithms is the optimal distributed solution which is computed offline given the complete knowledge about the data arrival process and classifier accuracies. 
%For simplicity, we focus on the distributed classification problem of classifier $i$ 
In the optimal classification scheme, for each context $x \in {\cal X}$ classifier $i$ wants to find the optimal classification function from the set $\cup_{i \in {\cal M}} {\cal F}_i$, i.e., the classification function $k$ with the highest accuracy minus the cost of classification $d_k$. We assume that the context space and classification accuracies have the following structural property:
%
\begin{assumption} \label{ass:lipschitz}
For each $k \in \cup_{i \in {\cal M}} {\cal F}_i$, there exists $L>0$, $\alpha>0$ such that for all $x,x' \in {\cal X}$
%
\begin{align*}
|\pi_k(x) - \pi_k(x')| \leq L |x-x'|^\alpha.
\end{align*}
%
\end{assumption}
%
Assumption \ref{ass:lipschitz} indicates that the accuracy of a classifier for similar contexts will be similar to each other. For example, when the context is the time of the day, population density which affects the classifier accuracy at times $x$ and $x'$ will be close to each other when the times $x$ and $x'$ are close to each other. Therefore the relation between classifier accuracy and time can be written down as a Lipschitz condition.  


\rev{For a set $A$ let $|A|$ denote the cardinality of that set.} In this section, we assume that the optimal classification scheme for any classifier $i$ 
partitions ${\cal X}$ into  $|\cup_{i \in {\cal M}} {\cal F}_i|$ sets in each of which a single classification function is optimal.
%Note that partitioning $[-1,1]^d$ is not enough because the noise can carry a data point outside of $[-1,1]^d$.
In order to solve this problem exactly, classifier $i$ needs to know the classification function that yields the \rev{lowest expected cost} for each $x \in {\cal X}$, which is computationally intractable. Assume for an instance that everything is known. Classifier $i$ has access to all classification functions $\cup_{i \in {\cal M}} {\cal F}_i$ and it knows $q_i$. Then the optimal solution for classifier $i$ is given by the following optimization problem.  
%
\begin{problem}\label{prob:opt}
When the classifier accuracies for each context $x \in {\cal X}$ is completely known, the optimal classification regions
%
\begin{align*}
{\cal R}^* = \{R^*_k\}_{(k \in \cup_{i \in {\cal M}} {\cal F}_i)},
\end{align*}
%
of ${\cal X}$ are the solution of 
%
\begin{align}
\textrm{{\bf (P1)  }} {\cal R}^* = \argmin_{{\cal R} \in \Theta} E \left[ \left| Y - \sum_{k \in \cup_{i \in {\cal M}} {\cal F}_i} k(X) I(X \in R_l) \right| + \sum_{k \in {\cal F}_i} d_k I(X \in R_k) + \sum_{k \in {\cal M}_{-i}}  d_k I \left(X \in \cup_{j \in {\cal F}_k} R_j \right)   \right], \label{eqn:opt}
\end{align}
%
where $\Theta$ is the set of $|\cup_{i \in {\cal M}} {\cal F}_i|$-set partitions of ${\cal X}$, the expectation is taken with respect to the distribution $q_i$ and $Y$ is the random variable denoting the true label. Here $I(X \in R_l)$ denotes the event that data received by the classifier belongs to the $l$th set of the partition ${\cal R}$ of ${\cal X}$.
%
\end{problem}

Note that ${\cal R}^*$ depends on $d_k$. Although, we made no assumptions on $d_k$s, in general exchanging data and label with other classifiers is more costly for a classifier then using its own classification function. Therefore without loss of generality we can assume that $d_l > d_k$ for $l \in {\cal M}_{-i}$, $k \in {\cal F}_i$.
%
The complexity of finding the optimal classification regions increases exponentially with $|\cup_{i \in {\cal M}} {\cal F}_i|$. The learning problem we are trying to solve is even harder because the classifiers are distributed, so each classifier cannot directly access to all classifier functions (classifier $i$ only knows set ${\cal F}_i$ and ${\cal M}$, but it does not know any ${\cal F}_j, j \in {\cal M}_{-i}$), and the distributions $q_i$, $i \in {\cal M}$ are unknown. Therefore, we need to use online learning techniques that does not rely on solving the optimization problem in given (\ref{eqn:opt}) or an estimated version of it. 

==> discussion.tex <==
\vspace{-0.1in}
\section{Discussion} \label{sec:discuss}
\vspace{-0.1in}

In this section we describe several extensions to our online learning algorithms and provide some application areas. In Table \ref{tab:compregret}, we summarize the regret results and memory requirements as well as our assumptions.

\remove{
\begin{table}[t]
\centering
{\fontsize{8}{8}\selectfont
\setlength{\tabcolsep}{.1em}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
& worst arrival  & worst arrival,   & best arrival, & best arrival  \\
&and correlation & best correlation & worst correlation& and correlation \\
\hline
CoS & $O \left(M F_{\max} T^{\frac{2\alpha+d}{3\alpha+d}} \right)$ 
& $O \left(|{\cal K}_i| T^{\frac{2\alpha+d}{3\alpha+d}} \right)$ 
& $O \left(M F_{\max}  T^{\frac{2\alpha}{3\alpha+d}} \right)$
& $O \left(|{\cal K}_i| T^{\frac{2\alpha}{3\alpha+d}} \right)$ \\
\hline
DDZA & $O \left(M F_{\max} T^{f_1(\alpha,d)}\right)$ 
& $O\left( |{\cal K}_i| T^{f_1(\alpha,d)}\right)$ 
& $O\left(M F_{\max} T^{2/3} \right)$ & $O\left(|{\cal K}_i| T^{2/3} \right)$ \\
\hline
\end{tabular}
}
\caption{Comparison CoS and DCZA}
\label{tab:compregret}
\end{table}
}
%
\add{
\begin{table}[t]
\centering
{\fontsize{7}{6}\selectfont
\setlength{\tabcolsep}{1em}
\begin{tabular}{|l|c|c|}
\hline
& CoS & DDZA \\
\hline
worst arrival & $O \left(M F_{\max} T^{\frac{2\alpha+d}{3\alpha+d}} \right)$ & $O \left(M F_{\max} T^{f_1(\alpha,d)}\right)$  \\
and correlation& & \\
\hline
worst arrival, & $O \left(|{\cal K}_i| T^{\frac{2\alpha+d}{3\alpha+d}} \right)$ & $O\left( |{\cal K}_i| T^{f_1(\alpha,d)}\right)$  \\
best correlation & & \\
\hline
best arrival,& $O \left(M F_{\max}  T^{\frac{2\alpha}{3\alpha+d}} \right)$ & $O\left(M F_{\max} T^{2/3} \right)$ \\
worst correlation&& \\
\hline
best arrival & $O \left(|{\cal K}_i| T^{\frac{2\alpha}{3\alpha+d}} \right)$ & $O\left(|{\cal K}_i| T^{2/3} \right)$ \\
and correlation & & \\
\hline
\end{tabular}
}
\caption{Comparison CoS and DDZA}
\label{tab:compregret}
\vspace{-0.4in}
\end{table}
}

\vspace{-0.2in}
\subsection{Exploration reduction by increasing memory} \label{sec:reduction}

Whenever a new level $l$ hypercube is activated at time $t$, DCZA spends at least $O(t^z \log t)$ time steps to explore the arms in that hypercube. The actual number of explorations can be reduced by increasing the memory of DCZA. Each active level $l$ hypercube splits into $2^d$ level $l+1$ hypercubes when the number of arrivals to that hypercube exceeds $A 2^{pl}$. Let the $l+1$ hypercubes formed by splitting of a level $l$ hypercube called {\em child} hypercubes. The idea is to keep $2^d$ sample mean estimates for each arm in each active level $l$ hypercube corresponding to its child level $l+1$ hypercubes, and to use the average of these sample means to exploit an arm when the level $l$ hypercube is active. Based on the arrival process to level $l$ hypercube, all level $l+1$ child hypercubes may have been explored more than $O(t^z \log t)$ times when they are activated. In the worst case, this guarantees that at least one level $l+1$ child hypercube is explored at least $A 2^{pl-d}$ times before being activated. The memory requirement of this modification is $2^d$ times the memory requirement of original DCZA, so in practice this modification is useful for $d$ small.  

\comment{
\subsection{Context to capture concept drift}

An important application in data classification systems is to capture the changes in the trends. Formally, concept is the whole distribution of the problem in a certain point of time \cite{narasimhamurthy2007framework}. Concept drift is a change in the distribution the problem \cite{gama2004learning, gao2007appropriate}. Examples of concept drift include recommender systems where the interests of users change over time and network security applications where the incoming and outgoing traffic patterns vary depending on the time of the day.

Researchers have categorized concept drift according to the properties of the drift. Two important metrics are the {\em severity} and the {\em speed} of the drift given in \cite{minku2010impact}. The severity is the amount of changes that the new concept causes, while the {\em speed} of a drift is how fast the new concept takes place of the old concept. 
%
Both of these categories can be captured by our contextual data mining framework. Given a final time $T$, let $x_t = t/T$ be the context. Thus $x_t \in [0,1]$ always. Then the Lipschitz condition given in Assumption \ref{ass:lipschitz2} can be rewritten as
%
\begin{align*}
|\pi_k(t) - \pi_k(t')| \leq \frac{L|t-t'|^\alpha}{T^\alpha}.
\end{align*} 
%
Here $L$ captures the severity while $\alpha$ captures the speed of the drift. Previous work on concept drift categorized the drift according to its severity, speed and several other metrics. Our distributed learning algorithms CoS and DCZA can both be used to address concept drift, and provide sublinear convergence rate to the optimal classification scheme, given by the results of Theorems \ref{theorem:cos} and \ref{thm:adaptivemain}, for $d=1$. 

Most of these work focused on incremental and online ensemble learning techniques with the goal of characterizing the advantage of ensemble diversity under concept drift. Some considered algorithms with drift detection mechanism \cite{baena2006early, minku2012ddd} while some others designed algorithms without a drift detection mechanism \cite{stanley2003learning, kolter2007dynamic}. A drift detection mechanism usually resets the learned parameters when a drift is detected and starts with a new set of parameters, while algorithms without a drift detection mechanism changes weights associated with the learners based on the change in the reward when a drift occurs.

However, to the best of our knowledge all the previous methods are develop in an ad-hoc basis with no provable performance guarantees. In this subsection, we showed how our distributed contextual learning framework can be used to obtain regret bounds for classification under concept drift. Our learning framework can be extended to ensemble learning by jointly updating the sample mean accuracies of classification functions and the weights of the ensemble learner. Although, the results from combinatorial bandit problems \cite{gai2012combinatorial} can be utilized to solve the online distributed contextual ensemble learning problem, design of an algorithm that jointly optimizes the accuracies and weights with sublinear regret with respect to the best ensemble learner is a complicated problem which is out of the scope of this paper. We aim to address this in our future work.

Two other important criteria to categorize concept drifts is {\em recurrence} \cite{narasimhamurthy2007framework} and {\em frequency} \cite{minku2010impact}. If the drift is recurrent, an old concept can replace the current concept at a future time. If the drift has a frequency $1/\tau$, then concept changes occur at every $\tau$ time steps. Moreover concept itself can also be recurrent, such as in rain forecast, where concepts have a high correlation with the month of the year. Both recurrence and frequency can be captured by our online learning framework. 
%
For example, assume that the concept is recurrent with period $\tau>0$. Knowing this, learner $i$ can run DCZA with context $x_t = t \mod \tau$. Therefore, the regret of bound of Theorem \ref{thm:adaptivemain} will hold with $d=1$. 
}
\vspace{-0.2in}
\subsection{Comparison with a centralized contextual bandit algorithm}

A zooming algorithm for the centralized contextual bandits is proposed in \cite{slivkins2009contextual}, which is called {\em contextual zooming algorithm} (CZA). This algorithm creates balls over the similarity space, which is the product of arm and context spaces, and at each time step chooses an active ball in which the context lies. Similar to DCZA when the number of arrivals to a ball exceeds some number, a new child ball with half the radius of the original ball is created centered at the most recent context. The authors provide $O(T^{(1+d_c)/(2+d_c)} \log T)$ upper bound on regret, where $d_c$ is a special number that is called the {\em zooming} dimension of the problem. Usually $d_c$ is smaller than the Euclidian dimension $d$. The dimension $d_c$ is computed by taking into account {\em benign} context arrivals and {\em benign} expected payoffs.
%
\rev{Here benign context arrivals means that the context arrivals which occur more frequently then others, and benign expected payoffs means that the payoffs of arms which are significantly higher than the payoffs of the other arms.}
%
For the worst-case, $d_c$ is equal to the dimension of the similarity space, which is $d+1$ for our case. Therefore the worst-case context arrival regret of CZA is $O(T^{(2+d)/(3+d)} \log T)$ which is equal to the regret of CoS for $\alpha=1$. While in the best-case context arrival, since for our problem dimension of the arm space is $1$, we have $d_c>1$, hence the best-case regret of CZA is greater than $O(T^{2/3}) \log T$ which is worse than DCZA. CZA cannot be applied to our distributed learning setting, because the created balls are centered around the last context arrival, whereas the position of the hypercubes in DCZA does not depend on the context arrival process. learner $i$, who have a level $l$ active hypercube that contains $x_t$ can safely call any learner $k$ which has a level $l' \geq l$ hypercube that contains $x_t$, for any future context which lies in the same level $l$ hypercube. Moreover checking which hypercube the context belongs is much simpler in DCZA than in CZA since we only need to compare the level of the active hypercubes that contains the coordinate $x_t$, while in CZA, the regions covered by each active ball should be scanned to find to which ball $x_t$ belongs. 
\vspace{-0.3in}
\subsection{Sending only the context but not the data}

We note that the communication cost of sending the data and receiving the prediction from another learner $k \in {\cal M}_{-i}$ is captured by the cost $d_k$. However, if $d_k$ is too high then in the optimal distributed solution given in (\ref{eqn:opt2}) that requires full data exchange, arm $k$ may not be selected for any $x_t \in {\cal X}$. In this case, algorithms CoS and DCZA will converge to the optimal solution that only uses the arms in ${\cal F}_i$. But is there a better way by which $i$ can exploit other good learners with smaller cost? One solution is that instead of sending the high dimensional data, $i$ can send the low dimensional context to learner $k$. In this way the cost of communication will be much smaller than $d_k$ and may even be less than the costs $d_j$, $j \in {\cal K}_i$. Then, learner $k$ will not actually classify but knowing the context, it will send back a prediction which has the highest percentage of being correct among all the predictions made by $k$ in the partition which the context belongs. This may outperform the optimal solution which requires full data exchange, especially if the prediction results of $k$ are strongly correlated with the context. Also, if there are privacy concerns, sending only the context information may be a better option.
\vspace{-0.2in}
\rmv{
\subsection{Cooperation among the learners}
In our analysis we assumed that learner $i$ can call any other learner $k \in {\cal M}_{-i}$ with a cost $d_k$, and $k \in {\cal M}_{-i}$ always sends back its prediction in the same time slot. However, learner $k$ also has to classify its own data stream thus it may not be possible for it to classify $i$s data without delay. We considered the effect of a bounded delay in Corollary \ref{cor:uniform}. 
%
We note that there is also a cost for learner $k$ associated with communicating with learner $i$, but it is small since learner $k$ only needs to send $i$ its prediction but not the data. However, even tough learner $k$ does not have immediate benefit from classifying $i$'s data, similar to $i$ it can use other learners to increase its prediction accuracy minus classification cost. In this paper we assumed that the learners are cooperative and there are no strategic interactions. Each learner should classify another learner's data when requested. This does not affect the optimal policy we derive for learner $i$ since the requests of other learner's is independent of actions of $i$.
}
%
%Dealing with strategic interactions is a future research topic.
% One way to ensure participation in classification of other's data is to use rating mechanisms.  
\comment{
\vspace{-0.1in}
\subsection{Context dependent costs}

In our analysis we assumed that classification cost $d_k$ is constant and does not depend on the context. In general this cost can be context or data dependent. 
%We assumed that the expected reward of choosing arm $k$ in context $x$ is equal to $\pi_k(x) - d_k$ for classifier $i$. 
For example, consider a network and two arms $l$ and $k$ for which $d_k >> d_l$ but $0<\pi_k(x) - \pi_l(x)<<1$. 
The network can go down when attacked at a specific context $x'$, thus, the expected loss $g_l(x')$ for arm $l$ can be much higher than the expected loss $g_k(x')$ for arm $k$. Then, in the optimal solution, arm $k$ will be chosen instead of arm $l$ even though $d_k >> d_l$.
%
Our results will hold for any general reward function $g_k(x)$ for which Assumption \ref{ass:lipschitz2} holds. 
}

==> zooming_scheme.tex <==
\vspace{-0.15in}
\section{A distributed adaptive context partitioning algorithm} \label{sec:zooming}

In most of the real-world applications of online distributed data mining, the data can be both temporally and spatially correlated and data arrival patterns can be non-uniform.
%
%\rev{For example, cyber-attacks in a network usually follow a bursty Markovian model where a long sequence of time slots with no attacks is followed by a long sequence of time slots with attacks (e.g., KDD Cup 1999 data set from UCI KDD archive).} 
% 
Intuitively it seems that the loss due to choosing a suboptimal arm for a context can be further minimized if the algorithm inspects the regions of space with large number of data (hence context) arrivals more carefully. Next, we do this by introducing the {\em distributed context zooming} algorithm (DCZA).

\vspace{-0.2in}
\subsection{The DCZA algorithm}

In the previous section the finite partition of hypercubes ${\cal P}_T$ is \rev{formed by CoS} at the beginning by choosing the slicing parameter $m_T$. \rev{Differently, DCZA} adaptively generates the partition by learning from the context arrivals. Similar to CoS, DCZA estimates the qualities of the arms for each set in the partition.
%
DCZA starts with a single hypercube which is the entire context space ${\cal X}$, then divides the space into finer regions and explores them as more data arrives. In this way, the algorithm focuses on parts of the space in which there is large number of data arrivals. 
%
The idea of zooming into the regions of context space with high arrivals is previously addressed in \cite{slivkins2009contextual} by activating balls with smaller radius over time. However, the results in \cite{slivkins2009contextual} cannot be generalized to a distributed setting because each learner may have different active balls for the same context at the same time. Our proposed algorithm uses a more structured zooming with hypercubes to address the distributed nature of our problem.
%
Basically, the learning algorithm for learner $i$ should zoom into the regions of space with large number of data arrivals, but it should also persuade other learners to zoom to the regions of the space where learner $i$ has a large number of data arrivals. The pseudocode of DCZA is given in Figure \ref{fig:DDZA}, and the training, exploration, exploitation and initialization modules are given in Figures \ref{fig:mtrain} and \ref{fig:minitialize}.

For simplicity, in this section let ${\cal X} = [0,1]^d$, which is known by all learners. In principle, DCZA will work for any ${\cal X}$ that is bounded given that DCZA knows a hypercube $C_U$ which covers ${\cal X}$, i.e., ${\cal X} \subset C_U$. We call a $d$-dimensional hypercube which has sides of length $2^{-l}$ a level $l$ hypercube. Denote the partition of ${\cal X}$ generated by level $l$ hypercubes by ${\cal P}_l$. We have $|{\cal P}_l| = 2^{ld}$. Let ${\cal P} := \cup_{l=0}^\infty {\cal P}_l$ denote the set of all possible hypercubes. Note that ${\cal P}_0$ contains only a single hypercube which is ${\cal X}$ itself. 
%
At each time step, DCZA keeps a set of hypercubes that cover the context space which are mutually exclusive. We call these hypercubes {\em active} hypercubes, and denote the set of active hypercubes at time $t$ by ${\cal A}_t$.  Clearly, we have $\cup_{C \in {\cal A}_t} C = {\cal X}$. Denote the active hypercube that contains $x_t$ by $C_t$. The arm chosen at time $t$ only depends on the previous observations and actions taken on $C_t$. 
%
Let $N^i_C(t)$ be the number of times context arrives to hypercube $C$ in learner $i$ by time $t$. Once activated, a level $l$ hypercube $C$ will stay active until the first time $t$ such that $N^i_C(t) \geq A 2^{pl}$, where $p>0$ and $A>0$ are parameters of DCZA. After that, DCZA will divide $C$ into $2^d$ level $l+1$ hypercubes. 

When context $x_t \in C \in {\cal A}_t$ arrives, DCZA either explores or exploits one of the arms in ${\cal K}_i$. Similar to CoS, for each arm in ${\cal F}_i$, DCZA have a single exploration control function $D_1(t)$, while for each arm in ${\cal M}_{-i}$, DCZA have training and exploration control functions $D_2(t)$ and $D_3(t)$ that controls when to train, explore or exploit. 
%
For an arm $k \in {\cal F}_i$, all the observations are used by learner $i$ to estimate the expected reward of that arm. This estimation is different for $k \in {\cal M}_{-i}$. This is because learner $i$ cannot choose the classification function that is used by learner $k$. If the estimated rewards of classification functions of learner $k$ are inaccurate, $i$'s estimate of $k$'s reward will be different from the expected reward of $k$'s optimal classification function. 
%
Therefore, learner $i$ uses the rewards from learner $k$ to estimate the expected reward of learner $k$ only if it believes that learner $k$ estimated the expected rewards of its own classification functions accurately. In order for learner $k$ to estimate the rewards of its own classification functions accurately, if the number of data arrivals to learner $k$ in set $C$ is small, learner $i$ {\em trains} learner $k$ by asking it to classify $i$'s data and returns the true label to learner $k$ to make it learn from its actions. 
%
In order to do this, learner $i$ keeps two counters $N^i_{1,k,C}(t)$ and $N^i_{2,k,C}(t)$, which are initially set to $0$. At the beginning of each time step for which $N^i_{1,k,C}(t) \leq D_2(t)$, learner $i$ asks $k$ to send it $N^k_C(t)$ which is the number of data arrivals to learner $k$ from the activation of $C$ to time $t$ including the data sent by learner $i$. If $C$ is not activated by $k$ yet, then it sends $N^k_C(t) = 0$ and activates the hypercube $C$. Then learner $i$ sets $N^i_{1,k,C}(t) = N^k_C(t) - N^i_{2,k,C}(t)$ and checks again if $N^i_{1,k,C}(t) \leq D_2(t)$. If so, then it trains learner $k$ and updates $N^i_{1,k,C}(t)$. If $N^i_{1,k,C}(t) > D_2(t)$, this means that learner $k$ is trained enough so it will almost always select its optimal classification function when called by $i$. Therefore, $i$ will only use observations when $N^i_{1,k,C}(t) > D_2(t)$ to estimate the expected reward of $k$. To have sufficient observations from $k$ before exploitation, $i$ explores $k$ when $N^i_{1,k,C}(t) > D_2(t)$ and $N^i_{2,k,C}(t) \leq D_3(t)$ and updates $N^i_{2,k,C}(t)$. For simplicity of notation we let $N^i_{k,c} := N^i_{2,k,C}(t)$ for $k \in {\cal M}_{-i}$.
%
Let
%
\begin{align*}
&{\cal S}^i_C(t) := \left\{ k \in {\cal F}_i \textrm{ such that } N^i_{k,C}(t) \leq D_1(t)  \textrm{ or } k \in {\cal M}_{-i} \right. \\
&\left. \textrm{ such that } N^i_{1,k,C}(t) \leq D_2(t) \textrm{ or } N^i_{2,k,C}(t) \leq D_3(t)   \right\}.
\end{align*} 
%
If $S^i_C(t) \neq \emptyset$ then DCZA randomly selects an arm in $S^i_C(t)$ to explore, while if $S^i_C(t) = \emptyset$, DCZA selects an arm in 
%
%\begin{align*}
$\argmax_{k \in {\cal K}_i} \bar{r}^i_{k,C_t}(t)$,
%\end{align*}
%
where $\bar{r}^i_{k,C_t}(t)$ is the sample mean of the rewards collected from arm $k$ in $C_t$ from the activation of $C_t$ to time $t$ for $k \in {\cal F}_i$, and it is the sample mean of the rewards collected from \rev{exploration and exploitation} steps of arm $k$ in $C_t$ from the activation of $C_t$ to time $t$ for $k \in {\cal M}_{-i}$.

\add{\vspace{-0.15in}}
\subsection{Analysis of the regret of DCZA}

We analyze the regret of DCZA under different context arrivals. In our first setting, we consider the worst-case scenario where there are no arrivals to learners other than $i$. In this case learner $i$ should train all the other learners in order to learn the optimal classification scheme. In our second setting, we consider the best scenario where data arrival to each learner is the same. In this case $i$ does not need to train other learners and the regret is much smaller. 
%Then in our third setting we introduce correlation between the classifiers and assume that at each time step data arriving to classifier $i$ and classifier $k$ will be same with probability $q_k$. 

We start with a simple lemma which gives an upper bound on the highest level hypercube that is active at any time $t$.
%
\begin{lemma}\label{lemma:levelbound}
All the active hypercubes ${\cal A}_t$ at time $t$ have at most a level of 
%
%\begin{align*}
$(\log_2 t)/p + 1$.
%\end{align*}
%
\end{lemma}
%
\remove{
\begin{proof}
Let $l+1$ be the level of the highest level active hypercube. We must have
%
\begin{align*}
A \sum_{j=0}^{l} 2^{pj} < t,
\end{align*}
otherwise the highest level active hypercube will be less than $l+1$. We have for $t/A >1$,
%
\begin{align*}
A \frac{2^{p(l+1)}-1}{2^p-1} < t
\Rightarrow 2^{pi} < \frac{t}{A} 
\Rightarrow i < \frac{\log_2 t}{p}.
\end{align*}
%
\end{proof}
}

In order to analyze the regret of DCZA, we first bound the regret in each level $l$ hypercube. We do this based on the worst-case and identical data arrival cases separately. The following lemma bounds the regret due to explorations in a level $l$ hypercube. 

\begin{lemma} \label{lemma:adapexplore}
Let $D_1(t) = D_3(t) =  t^z \log t $ and $D_2(t) = F_{\max} t^z \log t $. Then, for any level $l$ hypercube the regret due to explorations by time $t$ is bounded above by
%
\add{
$(|{\cal F}_i| + (M-1)(F_{\max} + 1)) (t^z \log t +1)$.
}
%
\remove{
\begin{align}
(|{\cal F}_i| + (M-1)(F_{\max} + 1)) (t^z \log t +1). \label{eqn:adapexplore1}
\end{align}
}
%
When the data arriving to each learner is identical and $|{\cal F}_i| \leq |{\cal F}_k|$, $k \in {\cal M}_{-i}$, regret due to explorations by time $t$ is bounded above by
%
\add{
$(|{\cal F}_i| + (M-1)) (t^z \log t +1)$.
}
\remove{
\begin{align}
(|{\cal F}_i| + (M-1)) (t^z \log t +1). \label{eqn:adapexplore2}
\end{align}
}
%
\end{lemma}
%
\remove{
\begin{proof}
The proof is similar to Lemma \ref{lemma:explorations}. Note that when the data arriving to each learner is the same and $|{\cal F}_i| \leq |{\cal F}_k|$, $k \in {\cal M}_{-i}$, we have $N^i_{1,k,C}(t) > D_2(t)$ for all $k \in {\cal M}_{-i}$ whenever $N^i_{j,C}(t) > D_1(t)$ for all $j \in {\cal F}_i$.
\end{proof}
}
%
\rev{From Lemma \ref{lemma:adapexplore}, the regret due to explorations increases exponentially with $z$ for each hypercube. 
}

For a level $l$ hypercube $C$, the set of suboptimal arms is given by
%
\vspace{-0.1in}
\begin{align*}
{\cal L}^i_{C,l,B} := \left\{ k \in {\cal K}_i :  \underline{\mu}_{k^*(C),C} - \overline{\mu}_{k,C} > B L d^{\alpha/2} 2^{-l \alpha} \right\},
\end{align*}
%
where $B>0$ is a constant.
%
In the next lemma we bound the regret due to choosing a suboptimal action in the exploitation steps in a level $l$ hypercube. 

\begin{lemma} \label{lemma:suboptimal}
Let ${\cal L}^i_{C,l,B}$, $B = 12/(L d^{\alpha/2}2^{-\alpha}) +2)$ denote the set of suboptimal actions for level $l$ hypercube $C$. When DCZA is run with parameters $p>0$, $2\alpha/p \leq z<1$, $D_1(t) = D_3(t) = t^z \log t$ and $D_2(t) = F_{\max} t^z \log t$, for any level $l$ hypercube $C$, the regret due to choosing suboptimal actions in exploitation steps, i.e., $E[R_{C,s}(T)]$, is bounded above by
%
\vspace{-0.1in}
\begin{align*}
4 \beta_2 |{\cal F}_i| + 8 (M-1) F_{\max} \beta_2 T^{z/2}/z.
\end{align*}
\vspace{-0.2in}
%
\end{lemma}
%
\remove{
\begin{proof}
The proof of this lemma is similar to the proof of Lemma \ref{lemma:suboptimal}, thus some steps are omitted.
Let $\Omega$ denote the space of all possible outcomes, and $w$ be a sample path. The event that the algorithm exploits in $C$ at time $t$ is given by
%
\begin{align*}
{\cal W}^i_{C}(t) := \{ w : S^i_{C}(t) = \emptyset, x_i(t) \in C, C \in {\cal A}_t  \}.
\end{align*}
%
Similar to the proof of Lemma \ref{lemma:suboptimal}, we will bound the probability that the algorithm chooses a suboptimal arm in an exploitation step in $C$, and then bound the expected number of times a suboptimal arm is chosen by the algorithm. Recall that loss in every step can be at most 2. Let ${\cal V}^i_{k,C}(t)$ be the event that a suboptimal action $k$ is chosen. Then
%
\begin{align*}
E[R_{C,s}(T)] \leq \sum_{t=1}^T \sum_{k \in {\cal L}^i_{C,l,B} } P({\cal V}^i_{k,C}(t), {\cal W}^i_{C}(t)).
\end{align*} 
%
Let ${\cal B}^i_{k,C}(t)$ be the event that at most $t^{\phi}$ samples in ${\cal E}^i_{k,C}(t)$ are collected from suboptimal classification functions of the $k$-th arm. Obviously for any $k \in {\cal F}_i$, ${\cal B}^i_{k,C}(t) = \Omega$, while this is not always true for $k \in {\cal M}_{-i}$. 
We have
% 
\begin{align}
P \left( {\cal V}^i_{k,C}(t), {\cal W}^i_{C}(t) \right) 
&\leq P \left( \bar{r}^{\textrm{b}}_{k,C}(N^i_{k,C}(t))
\geq \bar{r}^{\textrm{w}}_{k^*(C),C}(N^i_{k^*(C),C}(t))
-  2 t^{\phi-1} , 
\bar{r}^{\textrm{b}}_{k,l}(N^i_{k,C}(t)) < \overline{\mu}_{k,C} + L d^{\alpha/2} 2^{-l\alpha} \right. \notag \\
& \left. + H_t +  2 t^{\phi-1}, 
 \bar{r}^{\textrm{w}}_{k^*(C),C}(N^i_{k^*(C),C}(t)) > \underline{\mu}_{k^*(C),C} - L d^{\alpha/2} 2^{-l\alpha} - H_t,
{\cal W}^i_{C}(t)    \right). \label{eqn:makezero} \\
&+ P \left( \bar{r}^{\textrm{b}}_{k,C}(N^i_{k,C}(t)) \geq \overline{\mu}_{k,C} + H_t, {\cal W}^i_{C}(t) \right) \notag \\
&+ P \left( \bar{r}^{\textrm{w}}_{k^*(C),C}(N^i_{k^*(C),C}(t))  \leq \underline{\mu}_{k^*(C),C} - H_t + 2 t^{\phi-1}, {\cal W}^i_{C}(t) \right) \notag \\
&+ P(({\cal B}^i_{k,C}(t))^c), \notag
\end{align}
%
where $H_t >0$. In order to make the probability in (\ref{eqn:makezero}) equal to $0$, we need
%
\begin{align}
4 t^{\phi-1} + 2H_t \leq (B-2) L d^{\alpha/2} 2^{-l\alpha}. \label{eqn:adaptivecondition1}
\end{align}
%
By Lemma \ref{lemma:levelbound}, (\ref{eqn:adaptivecondition1}) holds when 
%
\begin{align}
4 t^{\phi-1} + 2H_t \leq (B-2) L d^{\alpha/2} 2^{-\alpha} t^{-\alpha/p}. \label{eqn:adaptivecondition2}
\end{align}
%
For $H_t = 4 t^{\phi-1}$, $\phi = 1 - z/2$, $z \geq 2\alpha/p$ and $B = 12/(L d^{\alpha/2}2^{-\alpha}) +2)$, (\ref{eqn:adaptivecondition2}) holds by which (\ref{eqn:makezero}) is equal to zero. Also by using a Chernoff-Hoeffding bound we can show that
%
\begin{align*}
P \left( \bar{r}^{\textrm{b}}_{k,C}(N^i_{k,C}(t)) \geq \overline{\mu}_{k,C} + H_t, {\cal W}^i_{C}(t) \right) \leq e^{-2 (16 \log t)} \leq \frac{1}{t^2},
\end{align*}
%
and
\begin{align*}
P \left( \bar{r}^{\textrm{w}}_{k^*(C),C}(N^i_{k^*(C),C}(t))  \leq \underline{\mu}_{k^*(C),C} - H_t + 2 t^{\phi-1}, {\cal W}^i_{C}(t) \right) \leq e^{-2 (4 \log t)} \leq \frac{1}{t^2}.
\end{align*}
%
We also have $P({\cal B}^i_{k,C}(t)^c)=0$ for $k \in {\cal F}_i$ and 
%
\begin{align*}
P({\cal B}^i_{k,C}(t)^c) &\leq \frac{E[X^i_{k,C}(t)]}{t^\phi} \\
& \leq 2 F_{\max} \beta_2 t^{z/2 - 1}.
\end{align*}
%
for $k \in {\cal M}_{-i}$, where $X^i_{k,C}(t)$ is the number of times a suboptimal classification function of learner $k$ is selected when learner $i$ calls $k$ in exploration and exploitation phases in an active hypercube $C$ by time $t$. Combining all of these we get
%
\begin{align*}
P \left( {\cal V}^i_{k,C}(t), {\cal W}^i_{C}(t) \right)  \leq \frac{2}{t^2},
\end{align*}
for $k \in {\cal F}_i$ and
\begin{align*}
P \left( {\cal V}^i_{k,C}(t), {\cal W}^i_{C}(t) \right)  \leq \frac{2}{t^2} + 2 F_{\max} \beta_2 t^{z/2 - 1},
\end{align*}
%
for $k \in {\cal M}_{-i}$. These together imply that
%
\begin{align*}
E[R_{C,s}(T)] \leq 4 \beta_2 |{\cal F}_i| + 8 (M-1) F_{\max} \beta_2 \frac{T^{z/2}}{z}.
\end{align*}
%
\end{proof}
}
%

\rev{From Lemma \ref{lemma:suboptimal}, we see that the regret due to explorations increases exponentially with $z$ for each hypercube. 
}
%
In the next lemma we bound the regret due to choosing near optimal arms in a level $l$ hypercube.
%
\begin{lemma}\label{lemma:adapnearopt}
${\cal L}^i_{C,l,B}$, $B = 12/(L d^{\alpha/2}2^{-\alpha}) +2)$ denote the set of suboptimal actions for level $l$ hypercube $C$. When DCZA is run with parameters $p>0$, $2\alpha/p \leq z<1$, $D_1(t) = D_3(t) = t^z \log t$ and $D_2(t) = F_{\max} t^z \log t$, for any level $l$ hypercube $C$, the regret due to choosing near optimal actions in exploitation steps, i.e., $E[R_{C,n}(T)]$, is bounded above by
%
\begin{align*}
A B L d^{\alpha/2} 2^{p-\alpha} T^{\frac{p-\alpha}{p}} + 2 (M-1) F_{\max} \beta_2
\end{align*}
\end{lemma}
%
\remove{
\begin{proof}
Consider a level $l$ hypercube $C$. Let $X^i_{k,C}(t)$ denote the random variable which is the number of times a suboptimal classification function for arm $k \in {\cal M}_{-i}$ is chosen in exploitation steps of $i$ when the context is in set $C \in {\cal A}_t$ by time $t$. Similar to the proof of Lemma \ref{lemma:callother}, we have
%
\begin{align*} 
E[X^i_{k,C}(t)] \leq 2 F_{\max} \beta_2.
\end{align*}
Thus when a near optimal $k \in {\cal M}_{-i}$ is chosen the contribution to the regret from suboptimal classification functions of $k$ is bounded by $4 F_{\max} \beta_2$. The one-step regret of any near optimal classification function of any near optimal $k \in {\cal M}_{-i}$ is bounded by $2 B L d^{\alpha/2} 2^{-l \alpha}$. The one-step regret of any near optimal classification function $k \in {\cal F}_{i}$ is bounded by $B L d^{\alpha/2} 2^{-l \alpha}$. Since $C$ remains active for at most $A 2^{pl}$ context arrivals, we have
%
\begin{align*}
E[R_{C,n}(T)] &\leq 2 A B L d^{\alpha/2} 2^{(p-\alpha)l} + 2 (M-1) F_{\max} \beta_2.
%&\leq A B L d^{\alpha/2} 2^{p-\alpha} T^{\frac{p-\alpha}{p}} + 2 (M-1) F_{\max} \beta_2,
\end{align*}
%
%where the last inequality follows from Lemma \ref{lemma:levelbound}.
\end{proof}
}
%
\rev{From Lemma \ref{lemma:adapnearopt}, we see that the regret due to choosing near optimal actions in each hypercube increses with the parameter $p$ that determines how much the hypercube will remain active, and decreases with $\alpha$.}

Next we combine the results from Lemmas \ref{lemma:adapexplore}, \ref{lemma:suboptimal} and \ref{lemma:adapnearopt}, to obtain our regret bounds. All these lemmas bound the regret for a single level $l$ hypercube. The bounds in Lemmas \ref{lemma:adapexplore} and \ref{lemma:suboptimal} are independent of the level of the hypercube, while the bound in Lemma \ref{lemma:adapnearopt} depends on the level of the hypercube. We can also derive a level independent bound for $E[R_{C,n}(T)]$, but we can get a tighter regret bound by using the level dependent regret bound. 
%
In order to get the desired regret bound, we need to consider how many hypercubes of each level is formed by DCZA up to time $T$. The number of such hypercubes explicitly depends on the data/context arrival process. We will give regret bounds for the best and worst case context processes. Let the worst case process be the one in which all data that arrived up to time $T$ is uniformly distributed inside the context space, with minimum distance between any two context samples being $T^{-1/d}$. Let the best case process be the one in which all data arrived up to time $T$ is located inside the same hypercube $C$ of level $(\log_2 T)/p +1$. Also let the worst case correlation between the learners be the one in which data only arrives to learner $i$, and the best case correlation between the learners be the one in which the same data arrives to all learners at the same time. The following theorem characterizes the regret under these four possible extreme cases.
%
\begin{theorem}\label{thm:adaptivemain}
Consider four cases. C1) worst arrival and correlation, C2) worst arrival, best correlation, C3) best arrival, worst correlation, C4) best arrival and correlation. Let ${\cal L}^i_{C,l,B}$, $B = 12/(L d^{\alpha/2}2^{-\alpha}) +2)$ denote the set of suboptimal actions for level $l$ hypercube $C$. When DCZA is run with parameters $p = \frac{3\alpha + \sqrt{9 \alpha^2 + 8 \alpha d}}{2}$, $z = 2\alpha/p <1$, $D_1(t) = D_3(t) = t^z \log t$ and $D_2(t) = F_{\max} t^z \log t$, the regret by time $T$ is upper bounded by
\vspace{-0.1in}
\begin{align*}
\textrm{ C1) } & T^{f_1(\alpha,d)} \left( 2 A B L d^{\alpha/2} 2^{d+p-\alpha} + 2^{2d} Z_i \log T   \right) \\
&+ T^{f_2(\alpha,d)}  2^{2d+3} (M-1) F_{\max} \beta_2 \\ 
&+ T^{f_3(\alpha,d)} 2^{2d} \left( 2 (M-1) F_{\max} \beta_2 + Z_i + 4 \beta_2 |{\cal F}|_i  \right), \\
\textrm{ C2) } & T^{f_1(\alpha,d)} \left( 2 A B L d^{\alpha/2} 2^{d+p-\alpha} + 2^{2d} |{\cal K}_i| \log T   \right) \\
&+ T^{f_2(\alpha,d)}  2^{2d+3} (M-1) F_{\max} \beta_2 \\
&+ T^{f_3(\alpha,d)} 2^{2d} \left( 2 (M-1) F_{\max} \beta_2 + |{\cal K}_i| + 4 \beta_2 |{\cal F}|_i  \right), \\
\textrm{ C3) } & T^{2/3} \left( Z_i \log T \frac{\log_2 T}{p} + 2 AB L d^{\alpha/2} \frac{2^{2(p-\alpha)}}{2^{p-\alpha} -1}  \right) \\ 
&+ T^{1/3} 12 (M-1) F_{\max} \beta_2 \left( \frac{\log_2 T}{p} + 1 \right) \\
&+ \left( Z_i + 4 \beta_2 |{\cal F}_i| + 2(M-1) F_{\max} \beta_2  \right) \left( \frac{\log_2 T}{p} + 1 \right), \\
\textrm{ C4) } & T^{2/3} \left( |{\cal K}_i| \log T \frac{\log_2 T}{p} + 2 AB L d^{\alpha/2} \frac{2^{2(p-\alpha)}}{2^{p-\alpha} -1}  \right) \\
&+ T^{1/3} 12 (M-1) F_{\max} \beta_2 \left( \frac{\log_2 T}{p} + 1 \right) \\
&+ \left( |{\cal K}_i| + 4 \beta_2 |{\cal F}_i| + 2(M-1) F_{\max} \beta_2  \right) \left( \frac{\log_2 T}{p} + 1 \right),
\end{align*}
%
where
\begin{align*}
& Z_i = |{\cal F}_i| + (M-1)(F_{\max}+1), \\
&f_1(\alpha,d) = \frac{d+ \frac{\alpha}{2} + \frac{\sqrt{9\alpha^2 + 8 \alpha d}}{2}}{d+ \frac{3\alpha}{2} + \frac{\sqrt{9\alpha^2 + 8 \alpha d}}{2}} \\
& f_2(\alpha,d) = \frac{d}{d+\frac{3\alpha+\sqrt{9\alpha^2 + 8 \alpha d}}{2}} + \frac{2\alpha}{3\alpha + \sqrt{9\alpha^2 + 8 \alpha d} } \\
& f_3(\alpha,d) = \frac{d}{d+\frac{3\alpha+\sqrt{9\alpha^2 + 8 \alpha d}}{2}}.
\end{align*}
%
For any $\alpha>0$, $d \geq 1$, we have $f_1(\alpha,d) > f_2(\alpha,d) > f_3(\alpha,d)$.
%
\end{theorem}
%
\add{\vspace{-0.1in}}
\begin{proof}
Consider C1. It can be shown that in the worst case the highest level hypercube has level at most $1+ \log_{2^{p+d}} T$. The total number of hypercubes is bounded by
%
\begin{align*}
\sum_{l=0}^{1+ \log_{2^{p+d}} T} 2^{dl} \leq 2^{2d} T^{\frac{d}{d+p}}.
\end{align*}
%
Using the result in Lemma \ref{lemma:adapnearopt}, we calculate the regret from choosing near optimal arms as
\remove{
\begin{align*}
E[R_n(T)] &\leq 2^{2d} T^{\frac{d}{d+p}} ( 2(M-1) F_{\max} \beta_2) 
+ 2 AB L d^{\alpha/2} \sum_{l=0}^{1+ \log_{2^{p+d}} T} 2^{(d+ p-\alpha)l}  \\
&\leq 2^{2d} T^{\frac{d}{d+p}} ( 2(M-1) F_{\max} \beta_2) + 2 AB L d^{\alpha/2} 2^{2(d+p-\alpha)} T^{\frac{d+p-\alpha}{d+p}}.
\end{align*}
}
\add{
\begin{align*}
&E[R_n(T)] 
\leq 2^{2d} T^{\frac{d}{d+p}} ( 2(M-1) F_{\max} \beta_2) \\
&+ 2 AB L d^{\alpha/2} 2^{2(d+p-\alpha)} T^{\frac{d+p-\alpha}{d+p}}.
\end{align*}
}
%
Since the number of hypercubes is $O(T^{\frac{d}{d+p}})$, regret due to explorations is $O(T^{\frac{d}{d+p} + z} \log_T)$, while regret due to suboptimal arm selections is $O(T^{\frac{d}{d+p} + z})$, for $z \geq 2 \alpha/p$. These three terms are balanced when $z=2\alpha/p$ and $\frac{d+p-\alpha}{d+p} =\frac{d}{d+p} + z$.  Solving for $p$ we get
%
\remove{
\begin{align*}
p = \frac{3\alpha + \sqrt{9 \alpha^2 + 8 \alpha d}}{2}.
\end{align*}
}
\add{
$p = (3\alpha + \sqrt{9 \alpha^2 + 8 \alpha d})/2$.
}
%
Substituting these parameters and summing up all the terms we get the regret bound
%
\add{
$O(T^{f_1(\alpha,d)})$.
}
\remove{
\begin{align*}
O \left( T^{\frac{d+\alpha/2+\sqrt{9\alpha^2 + 8 \alpha d}/2}{d+3 \alpha/2+\sqrt{9\alpha^2 + 8 \alpha d}/2}}  \right).
\end{align*}
}
%
Only difference of C2 form C1 is that the explorations is reduced to $|{\cal K}_i|(T^z \log T +1) 2^{2d} T^{\frac{d}{d+p}}$.
%
Consider C3. By Lemma \ref{lemma:levelbound}, the number of activated hypercubes is upper bounded by $\log_2 T/p +1$, and by the property of context arrivals all the activated hypercubes have different levels. Using the result in Lemma \ref{lemma:adapnearopt}, we calculate the regret from choosing near optimal arms as
%
\add{
\begin{align*}
E[R_n(T)] 
&\leq \left( \frac{log_2 T}{p}+1 \right) ( 2(M-1) F_{\max} \beta_2) \\
&+ 2 AB L d^{\alpha/2} \frac{2^{2(p-\alpha)}}{2^{p-\alpha}} T^{\frac{p-\alpha}{p}}.
\end{align*}
}
\remove{
\begin{align*}
E[R_n(T)] &\leq \left( \frac{log_2 T}{p}+1 \right) ( 2(M-1) F_{\max} \beta_2) 
+ 2 AB L d^{\alpha/2} \sum_{l=0}^{\log_2 T/p +1} 2^{(p-\alpha)l}  \\
&\leq \left( \frac{log_2 T}{p}+1 \right) ( 2(M-1) F_{\max} \beta_2) + 2 AB L d^{\alpha/2} \frac{2^{2(p-\alpha)}}{2^{p-\alpha}} T^{\frac{p-\alpha}{p}}.
\end{align*}
}
%
Since there are at most $\log_2 T/p +1$ hypercubes by time $T$, the regret due to explorations and suboptimal arms are bounded by multiplying the regret results in Lemmas \ref{lemma:adapexplore} and \ref{lemma:suboptimal} with $\log_2 T/p +1$. All these terms are balanced by setting $z = 2\alpha/p$, $p=3\alpha$. Summing all the terms, we get the desired regret bound. 
%
Only difference of C4 form C3 is that the explorations is reduced to $|{\cal K}_i|(T^z \log T +1) (\log_2 T/p + 1)$.
\end{proof}

\vspace{-0.1in}
For the worst case arrivals C1 and C2, the time parameter of the regret approaches linear as $d$ increases. This is intuitive since the gains of zooming diminish when data is not concentrated in a region of space. The regret order of DCZA is 
%
\vspace{-0.2in}
\begin{align*}
O \left( T^{\frac{d+\alpha/2+\sqrt{9\alpha^2 + 8 \alpha d}/2}{d+3 \alpha/2+\sqrt{9\alpha^2 + 8 \alpha d}/2}}  \right),
\end{align*}
%
while the regret order of CoS is
%
\vspace{-0.1in}
\begin{align*}
O \left( T^{\frac{d+2\alpha}{d+3 \alpha}}  \right) = 
O \left( T^{\frac{d+\alpha/2+\sqrt{9\alpha^2}/2}{d+3 \alpha/2+\sqrt{9\alpha^2}/2}}  \right).
\end{align*}
%
This is intuitive since CoS is designed to capture the worst-case arrival process by forming a uniform partition over the context space, while DCZA adaptively learns over time that the best partition over the context space is a uniform one. The difference in the regret order between DCZA and CoS is due to the fact that DCZA starts with a single hypercube and splits it over time to reach the uniform partition which is optimal for the worst case arrival process, while CoS starts with the uniform partition at the beginning. Note that for $\alpha d$ small, the regret order of DCZA is very close to the regret order of CoS.
%
For C2 which is the best correlation case, the constant that multiplies the highest order term is $|{\cal K}_i|$, while for C1 which is the worst correlation case this constant is $|{\cal F}_i| (M-1) (F_{\max}+1)$ which is much larger. The regret of any intermediate level correlation will lie between these two extremes. 
%
For the best case arrivals C3 and C4, the time parameter of the regret does not depend on the dimension of the problem $d$. The regret is $O(T^{2/3})$ up to a logarithmic factor independent of $d$, which is always better than the $O(T^{(d+2\alpha)/(d+3\alpha)})$ bound of CoS. The difference between the regret terms of C3 and C4 is similar to the difference between C1 and C2.

Next, we assess the computation and memory requirements of DCZA and compare it with CoS. DCZA needs to keep the sample mean reward estimates of ${\cal K}_i$ arms for each active hypercube. A level $l$ active hypercube becomes inactive if the context arrivals to that hypercube exceeds $A 2^{pl}$. Because of this, the number of active hypercubes at any time $T$ may be much smaller than the number of activated hypercubes by time $T$.
%
For cases C1 and C2, the maximum number of activated hypercubes is $O(|{\cal K}_i| T^{\frac{d}{d+(3\alpha + \sqrt{9\alpha^2+8\alpha})/2}})$, while for any $d$ and $\alpha$, the memory requirement of CoS is upper bounded by $O(|{\cal K}_i| T^{d/(d+3\alpha)})$. This means that based on the data arrival process, the memory requirement of DCZA can be higher than CoS. 
However, since DCZA only have to keep the estimates of rewards in currently active hypercubes, but not all activated hypercubes, in reality the memory requirement of DCZA can be much smaller than CoS which requires to keep the estimates for every hypercube at all times. Under the best case data arrival given in C3 and C4, at any time step there is only a single active hypercube. Therefore, the memory requirement of DCZA is only $O({\cal K}_i)$, which is much better than CoS. Finally DCZA does not require final time $T$ as in input while CoS requires it. Although CoS can be combined with the doubling trick to make it independent of $T$, the constants that multiply the time order of regret will be large.



\add{\vspace{-0.1in}}
\begin{figure}[htb]
\fbox {
\begin{minipage}{0.95\columnwidth}
{\fontsize{8}{7}\selectfont
\flushleft{Distributed Context Zooming Algorithm (for learner $i$):}
\begin{algorithmic}[1]
\STATE{Input: $D_1(t)$, $D_2(t)$, $D_3(t)$, $p$, $A$}
\STATE{Initialization: ${\cal A} = \{[0,1]^d\}$, Run {\bf Initialize}(${\cal A}$)}
\STATE{Notation: $\boldsymbol{M}^i_C := (N^i_{k,c})_{k \in {\cal K}_i}$, 
$\bar{\boldsymbol{r}}_C := (\bar{r}_{k,C})_{k \in {\cal K}_i}$, $l_C$: level of hypercube $C$.}
\WHILE{$t \geq 1$}
\FOR{$C \in {\cal A}$}
\IF{$x_i(t) \in C$}
\IF{$\exists k \in {\cal F}_i \textrm{ such that } N^i_{k,C} \leq D_1(t)$}
\STATE{Run {\bf Explore}($k$, $N^i_{k,C}$, $\bar{r}_{k,C}$)}
\ELSIF{$\exists k \in {\cal M}_{-i} \textrm{ such that } N^i_{1,k,C} \leq D_2(t)$}
\STATE{Obtain $N^k_C(t)$ from $k$}
\IF{$N^k_C(t)=0$}
\STATE{ask $k$ to create hypercube $C$, set $N^i_{1,k,C}=0$}
\ELSE
\STATE{set $N^i_{1,k,C} = N^k_C(t) - N^i_{k,C}$}
\ENDIF
\IF{$N^i_{1,k,C} \leq D_2(t)$}
\STATE{Run {\bf Train}($k$, $N^i_{1,k,C}$)}
\ELSE
\STATE{Go to line 21}
%\STATE{Training phase: select arm $k$}
%\STATE{Receive reward $r_k(t) = I(k(x_i(t)) = y_t) - d_{k(x_i(t))}$}
%\STATE{$N^i_{1,k,C}++$}
\ENDIF
\ELSIF{$\exists k \in {\cal M}_{-i} \textrm{ such that } N^i_{k,C} \leq D_3(t)$}
\STATE{Run {\bf Explore}($k$, $N^i_{k,C}$, $\bar{r}_{k,C}$)}
%\STATE{Exploration phase: select arm $k$}
%\STATE{Receive reward $r_k(t) = I(k(x_i(t)) = y_t) - d_{k(x_i(t))}$}
%\STATE{$\bar{r}_{k,C} = \frac{N^i_{k,C} \bar{r}_{k,C} + r_k(t)}{N^i_{k,C} + 1}$}
%\STATE{$N^i_{k,C}++$}
\ELSE
\STATE{Run {\bf Exploit}($\boldsymbol{M}^i_C$, $\bar{\boldsymbol{r}}_C$, ${\cal K}_i$)}
%\STATE{Exploitation phase: select arm $k\in \argmax_{j \in {\cal K}_i} \bar{r}^i_{j,C}$}
%\STATE{Receive reward $r_k(t) = I(k(x_i(t)) = y_t) - d_{k(x_i(t))}$}
%\STATE{$\bar{r}_{k,C} = \frac{N^i_{k,C} \bar{r}_{k,C} + r_k(t)}{N^i_{k,C} + 1}$}
%\STATE{$N^i_{k,C}++$}
\ENDIF
\ENDIF
\STATE{$N^i_C = N^i_C +1$}
\IF{$N^i_C \geq A 2^{pl_C}$}
\STATE{Create $2^d$ level $l+1$ child hypercubes denoted by ${\cal A}^{l+1}_C$}
\STATE{Run {\bf Initialize}(${\cal A}^{l+1}_C$)}
\STATE{${\cal A} = {\cal A} \cup {\cal A}^{l+1}_C - C$}
\ENDIF
\ENDFOR
\STATE{$t=t+1$}
\ENDWHILE
\end{algorithmic}
}
\end{minipage}
} \caption{Pseudocode of the DCZA algorithm} \label{fig:DDZA}
\vspace{-0.3in}
\end{figure}



\begin{figure}[htb]
\fbox {
\begin{minipage}{0.95\columnwidth}
{\fontsize{8}{7}\selectfont
{\bf Initialize}(${\cal B}$):
\begin{algorithmic}[1]
\FOR{$C \in {\cal B}$}
\STATE{Set $N^i_C = 0$, $N^i_{k,C}=0$, $\bar{r}_{k,C}=0$ for $C \in {\cal A}, k \in {\cal K}_i$, $N^i_{1,k,C}=0$ for $k \in {\cal M}_{-i}$}
\ENDFOR
\end{algorithmic}
}
\end{minipage}
} \caption{Pseudocode of the initialization module} \label{fig:minitialize}
\add{\vspace{-0.23in}}
\end{figure}



